The Complexity of Pacing for Second-Price Auctions

Budget constraints are ubiquitous in online advertisement auctions. To manage these constraints and smooth out the expenditure across auctions, the bidders (or the platform on behalf of them) often employ pacing: each bidder is assigned a pacing multiplier between zero and one, and her bid on each item is multiplicatively scaled down by the pacing multiplier. This naturally gives rise to a game in which each bidder strategically selects a multiplier. The appropriate notion of equilibrium in this game is known as a pacing equilibrium. In this work, we show that the problem of finding an approximate pacing equilibrium is PPAD-complete for second-price auctions. This resolves an open question of Conitzer et al. [2021]. As a consequence of our hardness result, we show that the tatonnement-style budget-management dynamics introduced by Borgs et al. [2007] are unlikely to converge efficiently for repeated second-price auctions. This disproves a conjecture by Borgs et al. [2007], under the assumption that the complexity class PPAD is not equal to P. Our hardness result also implies the existence of a refinement of supply-aware market equilibria which is hard to compute with simple linear utilities.

==> Old_Proofs.tex <==
\section{Hardness - OLD}


We will prove the PPAD hardness of finding a pacing equilibrium in a MPPG by constructing a reduction from BIMATRIX.

\begin{definition}
    A two player normal form game specified by $n \times n$ payoff matrices $(A,B)$ is called normalized if $-1 \leq A_{ij},B_{ij} \leq 1$ for all $1 \leq i,j\leq n$.
\end{definition}

\begin{definition}
    Let $\Delta_n \coloneqq \{x \in \mathbb{R}^n \mid \sum_{i=1}^n x_ i =1, x_i \geq 0\}$ be the probability simplex in $n-1$ dimensions. $(x,y) \in \Delta_n^2$ is a Nash equilibrium of the game $(A,B)$ if for all $i,j \in [n]$,
    \begin{align*}
        A_iy - A_j y > 0 \implies x_j = 0 \quad \textrm{ and } \quad x^T B_i - x^T B_j > 0 \implies y_j = 0
    \end{align*}
\end{definition} 

BIMATRIX denotes the following problem: Given a $n \times n$ normalized two player game $(A,B)$, find a Nash equilibrium. The following result is known.
 
\begin{theorem}
    BIMATRIX is PPAD complete.
\end{theorem}

\subsection{Construction of the Second Price Pacing Game}
In this section, starting from an instance of the BIMATRIX problem $(A,B)$, we will construct a Mixed Price Pacing Game $\mathcal{S}$ such that every pacing equilibrium in $\mathcal{S}$ corresponds to a Nash equilibrium in the BIMATRIX game $(A,B)$.\\

Let $n$ be the number of strategies in the given instance of BIMATRIX. $\mathcal{S}$ consists of the following goods,
\begin{itemize}
    \item For player $i \in \{1,2\}$, there are
        \begin{itemize}
            \item $n$ probability goods, denoted by $\{G(i)_1, \dots, G(i)_n\}$
            \item $n$ auxiliary goods, denoted by $\{A(i)_1, \dots, A(i)_n\}$
            \item $1$ first price good, denoted by $L(i)$
        \end{itemize} 
    \item For each $p,q \in [n]$ and player $i \in \{1,2\}$, there are
        \begin{itemize}
            \item $n$ comparison goods, denoted by $\{C(i)^{p,q}_1, \dots, C(i)^{p,q}_n\}$
            \item $1$ dummy good, denoted by $D(i)^{p,q}$
            \item $1$ pacing good, denoted by $R(i)^{p,q}$
            \item $3$ enforcement goods, denoted by $\{E(i)_1^{p,q}, E(i)_2^{p,q}, E(i)_3^{p,q}\}$
        \end{itemize}
\end{itemize}

The first price goods, $\{F(1),F(2)\}$, follow the first price pricing rule and all other goods follow the second price pricing rule.\\

Set $c = \frac{1}{2n}$, $d = 1/4$ and $M = 8n^3$. In the description given below, an agent is called \emph{restricted} if she has non-zero value for exactly one good and has an infinite budget. The constructed instance, $\mathcal{S}$, has the following agents
\begin{itemize}
    \item For each player $i \in \{1,2\}$, there are
        \begin{itemize}
            \item $n$ probability agents, denoted by $\{P(i)_1, \dots, P(i)_n\}$. Agent $P(i)_j$ has budget $B(P(i)_j) = 3c/4$ and has non-zero value only for the following goods
                \begin{itemize}
                    \item $j$th probability good corresponding to player $i$ at  $v(P(i)_j, G(i)_j) = 1$
                    \item $j$th auxiliary good corresponding to player $i$ at $v(P(i)_j, A(i)_j) = 1$
                    \item $j$th comparison good corresponding to player $k \in \{1,2\}\setminus\{i\}$ and strategy pair $(p,q)$ at
                    \begin{align*}
                        v(P(i)_j, C(k)_j^{p,q}) =
                        \begin{cases}
                            B_{jp} - B_{jq} + 2 & \textrm{ if } i=1\\
                            A_{pj} - A_{qj} + 2 & \textrm{ if } i=2
                        \end{cases}
                    \end{align*}
                    for all strategy pairs $p,q \in [n]$ 
                    \item $3$rd enforcement good corresponding to player $i$ and strategy pair $(p,j)$ at $v(P(i)_j, E(i)^{p,j}_3) =1$ for every strategy $p \in [n]$
                \end{itemize}
            \item $1$ first price agent, denoted by $K(i)$, with budget $B(K(i)) = 2(n+1)$, who has non-zero value for only the following goods:
                \begin{itemize}
                    \item $j$th probability good $G(i)_j$ at $v(K(i), G(i)_j) = 4(n+1)$
                    \item first price good $L(i)$ at $v(K(i),L(i)) = 4(n+1)$
                    \item dummy good corresponding to player $k \in \{1,2\}\setminus\{i\}$ and strategy pair $(p,q)$ at $v(K(i), D(k)^{p,q}) = 8(n+1)$
                \end{itemize}
            
        \end{itemize}
        
    \item For each probability good $G(i)_j$, there is a restricted agent, denoted by $a(G(i)_j)$, with budget $\infty$, who values probability good $j$ at $v(a(G(i)_j), G(i)_j) = c$ and does not value any other good
    
    \item For each auxiliary good $A(i)_j$, there is a restricted agent, denoted by $a(A(i)_j)$, with budget $\infty$, who values probability good $j$ at $v(a(A(i)_j), A(i)_j) = c/2$ and does not value any other good
    
    \item For each player $i$ and strategy pair $p,q \in [n]$, there is a pacing agent, denoted by $Q(i)^{p,q}$, with budget
    \begin{align*}
        B(Q(i)^{p,q}) =
            \begin{cases}
                4(n+1) + M + c \sum_{j=1}^n [A_{pj} - A_{qj}] & \textrm{ if } i=1\\
                4(n+1) + M + c \sum_{j=1}^n [B_{jp} - B_{jq}] & \textrm{ if } i=2
            \end{cases}
    \end{align*}
    who has non-zero value only for the following goods
    \begin{itemize}
        \item comparison good $C(i)_j^{p,q}$ at $v(Q(i)^{p,q}, C(i)_j^{p,q}) = 4M$ for all $j \in [n]$
        \item dummy good $D(i)^{p,q}$ at $v(Q(i)^{p,q}, D(i)^{p,q}) = 4M$
        \item pacing good $R(i)^{p,q}$ at $v(Q(i)^{p,q}, R(i)^{p,q}) = 4M$
        \item enforcement good $E(i)_1^{p,q}$ at $v(Q(i)^{p,q}, E(i)_1^{p,q}) = d$
    \end{itemize}
    
    \item For each comparison good $C(i)_j^{p,q}$, there is a restricted agent, denoted by $a(C(i)_j^{p,q})$, with budget $\infty$, who values comparison good $C(i)_j^{p,q}$ at 
    \begin{align*}
                        v(a(P(i)^{p,q}), C(i)_j^{p,q}) =
                        \begin{cases}
                            c[A_{pj} - A_{qj} + 2] & \textrm{ if } i=1\\
                            c[B_{jp} - B_{jq} + 2] & \textrm{ if } i=2
                        \end{cases}
                    \end{align*}
    and does not value any other good
    \item For each pacing good $R(i)^{p,q}$, there is a restricted agent, denoted by $a(R(i)^{p,q})$, with budget $\infty$, who values pacing good $R(i)^{p,q}$ at $v(a(R(i)^{p,q}), R(i)^{p,q}) = M$ and does not value any other good
    \item For each player $i \in \{1,2\}$ and strategy pair $p,q \in [n]$, there is an enforcement agent, denoted by $F(i)^{p,q}$, with budget $B(F(i)^{p,q}) = 5d/4$, who has non-zero value only for the following goods
    \begin{itemize}
        \item enforcement good $E(i)_1^{p,q}$ at $v(F(i)^{p,q}, E(i)_1^{p,q}) =1$
        \item enforcement good $E(i)_2^{p,q}$ at $v(F(i)^{p,q}, E(i)_2^{p,q}) =d$
        \item enforcement good $E(i)_3^{p,q}$ at $v(F(i)^{p,q}, E(i)_3^{p,q}) =\frac{c}{2n}$
    \end{itemize}
    \item For each enforcement good $E(i)_2^{p,q}$, there is a restricted agent, denoted by $a(E(i)_2^{p,q})$, with budget $\infty$, who value the enforcement good $E(i)_2^{p,q}$ at $v(a(E(i)_2^{p,q}),E(i)_2^{p,q}) = d/2$ and does not value any other good
\end{itemize}

Now, starting from a pacing equilibrium of the constructed instance, we will find a solution to the given BIMATRIX instance. Consider any pacing equilibrium of $\mathcal{S}$, say $(\alpha, x)$. Define
\begin{align*}
    x_j = \frac{\max\{\alpha(P(1)_j) - c, 0\}}{\sum_{k=1}^n \max\{\alpha(P(1)_k) - c, 0\}}  \quad \textrm{ and } \quad y_j = \frac{\max\{\alpha(P(2)_j) - c, 0\}}{\sum_{k=1}^n \max\{\alpha(P(2)_k) - c, 0\}} \quad \textrm{for all } j \in [n]
\end{align*}

\textcolor{red}{NOTE: Separately consider the case when the denominator is 0}\\

Let $p,q \in [n]$ be strategies of player $1$ such that $A_p y - A_q y > 0$.\\

Observe that, in any pacing equilibrium, all the agents with infinite budget will have their pacing multiplier set to $1$.

\begin{claim}
    The following statements hold under $(\alpha, x)$:
    \begin{enumerate}
        \item For $i \in \{1,2\}$ and $p,q \in [n]$, $\alpha(Q(i)^{p,q}) \geq 1/4$
        \item For $i \in \{1,2\}$, $\alpha(K(i)) \geq 1/2(n+1)$
        \item For $i \in \{1,2\}$ and $j \in [n]$, $\alpha(P(i)_j) \geq c/2$
        \item For $i \in \{1,2\}$ and $p,q \in [n]$, $\alpha(F(i)^{p,q}) \geq 1/2$
        
    \end{enumerate}
\end{claim}
\begin{proof}
    \begin{enumerate}
        \item Suppose $\alpha(Q(i)^{p,q})< 1/4$. Then, the total expenditure of agent $Q(i)^{p,q}$ is no greater than $16n + d$ because $Q(i)^{p,q}$ does not win any part of the good $R(i)^{p,q}$. This contradicts the definition of a pacing equilibrium as $Q(i)^{p,q}$ is paced and $B(Q(i)^{p,q}) \geq M$. Hence, $\alpha(Q(i)^{p,q})\geq 1/n$.
        
        \item Suppose $\alpha(K(i)) < 1/2(n+1)$. Then, the total expenditure of $K(i)$ is no greater than $n + 2$ because, from (1), we get that $K(i)$ does not win any part of $D(i)^{p,q}_3$ for any $p,q \in [n]$. This contradicts the definition of a pacing equilibrium as $L(i)$ is paced and $B(K(i)) = 2(n+1)$. Hence, $\alpha(F(i)^{p,q}) \geq 1/2$.
        
        \item Suppose $\alpha(P(i)_j)< c/2$. Then, the total expenditure of $P(i)_j$ is no greater than $c/2$ because, using (2), we get that $P(i)_j$ does not win any part of $G(i)_j$ and $A(i)_j$. This is contradicts the definition of a pacing equilibrium as $P(i)_j$ is paced and $B(P(i)_j) = 3c/4$. Hence, $\alpha(P(i)_j) \geq c/2$.
        
        \item Suppose $\alpha(F(i)^{p,q}) < 1/2$. Then, the total expenditure of $F(i)^{p,q}$ is no greater than $d$ because, from (1), we get that $F(i)^{p,q}$ does not win any part of $E(i)^{p,q}_2$ and $E(i)^{p,q}_3$. This contradicts the definition of a pacing equilibrium as $F(i)^{p,q}$ is paced and $B(F(i)^{p,q}) = 5d/4$. Hence, $\alpha(F(i)^{p,q}) \geq 1/2$.
    \end{enumerate}
\end{proof}

\begin{claim}
    For $i \in \{1,2\}$, the first price agent, $K(i)$, is paced i.e. $\alpha(K(i) < 1$ and moreover, $$4\alpha(K(i)) (n+1) + \sum_{j = 1}^n \max\{\alpha_j, c\} = 2(n+1)$$
\end{claim}
\begin{proof}
    Suppose $\alpha(i) = 1$, then agent $K(i)$ spends $4(n+1)$ on the first price good, $L(i)$. This is a contradiction as $B(K(i)) = 2(n+1)$. Hence, $\alpha(K(i)) < 1$ and therefore, from the definition of pacing equilibrium, we get that the total expenditure of $K(i)$ is $2(n+1)$. Using claim 1, we get that $K(i)$ wins all of the probability goods $\{P(i)_1,\dots,P(i)_n\}$ and the first price good $F(i)$. Furthermore, she does not win any part of any other good. Therefore,
    \begin{align*}
        \alpha(K(i))\ [4(n+1)] + \sum_{j=1}^n \max\{\alpha_j, c\} = 2(n+1)
    \end{align*}
\end{proof}

Recall that $p,q \in [n]$ are strategies of player $1$ such that $A_p y - A_q y > 0$. Using the definition of $y$, we get that
\begin{align*}
    &A_p y - A_q y > 0\\
    \implies &\sum_{j=1}^n [A_{pj} - A_{qj}] y_j > 0\\
    \implies &\sum_{j=1}^n [A_{pj} - A_{qj}]\frac{\max\{\alpha(P(2)_j) - c, 0\}}{\sum_{k=1}^n \max\{\alpha(P(2)_k) - c, 0\}}  > 0\\
    \implies &\sum_{j=1}^n [A_{pj} - A_{qj}]\max\{\alpha(P(2)_j) - c, 0\}  > 0
\end{align*}

\begin{claim}
    $\alpha(Q(1)^{p,q}) = 1/4$
\end{claim}
\begin{proof}
    Suppose not. Then, from claim 1, we get that $\alpha(Q(1)^{p,q}) > 1/4$ and the total expenditure of agent $Q(1)^{p,q}$ is given by
    \begin{align*}
        &M + 8\alpha(K(2))(n+1) + \sum_{j=1}^n \max\{\alpha(P(2)_j)[2 + A_{pj} - A_{qj}], c[2 + A_{pj} - A_{qj}]\}\\
        =\ &M + 8\alpha(K(2))(n+1) + 2 \sum_{j=1}^n \max\{\alpha(P(2)_j, c\} + c \sum_{j=1}^n [A_{pj} - A_{qj}] + \sum_{j=1}^n \max\{\alpha(P(2)_j) - c, 0\} [A_{pj} - A_{qj}]\\
        =\ &M + 4(n+1) + c \sum_{j=1}^n [A_{pj} - A_{qj}] + \sum_{j=1}^n \max\{\alpha(P(2)_j) - c, 0\} [A_{pj} - A_{qj}]\\
        >\ &M + 4(n+1) + c \sum_{j=1}^n [A_{pj} - A_{qj}]\\
        =\ & B(Q(1)^{p,q})
    \end{align*}
    where the second equality follows from claim 2, and the inequality follows from the assumption that $A_p y - A_q y > 0$ and the definition of $y$. This is a contradiction and hence, using claim 1, we get that $\alpha(Q(1)^{p,q}) = 1/4$.
\end{proof}

\begin{claim}
    $\alpha(F(1)^{p,q}) = 1$
\end{claim}
\begin{proof}
    Using, claim 3, we get that agent $F(1)^{p,q}$ wins the enforcement good $E(1)^{p,q}$ at price $d/4$. Using, claim 1, she wins no part of enforcement good $E(1)^{p,q}$. Hence, her total expenditure can be no greater than $3d/4$. Therefore, the claim holds.
\end{proof}

\begin{claim}
    $x_q \coloneqq \frac{\max\{\alpha(P(1)_q) - c, 0\}}{\sum_{k=1}^n \max\{\alpha(P(1)_k) - c, 0\}} = 0$
\end{claim}
\begin{proof}
    Suppose $\max\{\alpha(P(1)_q) - c, 0\} > 0$ i.e. $\alpha(P(1)_q) > c$. Using the above claims, we get that the total expenditure of agent $P(1)_q$ is greater than $\frac{c}{4n}(n-1) + \frac{c}{2n} + c/2 > 3c/4$. Contradiction. Hence, the claim holds.
\end{proof}



==> competitive_equilibria.tex <==
\section{Relationship to Competitive Equilibrium}
We consider a single-slot auction market in which a set of bidders $N = \{1,, n\}$ target a set of goods $M = \{1,...,m\}$. Each bidder $i$ has a valuation $v_{ij} \geq 0$ for each good $j$, and a budget $B_i > 0$ to be spent across all goods. We assume that the goods are sold through independent (single slot) auctions where the highest bidder wins the good (the good can be shared if there are ties) and the payment is decided using pricing rule $p_j$ for good $j$ (which may be different for each item), and the valuations and budgets are assumed to be known to the auctioneer. Bidders receive a utility equal to the valuation of the goods for the auctions they win, minus the payments resulting from the auctions. If their payments exceed their budgets, they are assumed to receive a $-\infty$ utility.\\

The goal is to compute a vector of pacing multipliers that smooths out the spending of each bidder such that they stay within budget. A pacing multiplier for a bidder $i$ is a real number $\alpha_i \in [0, 1]$ that is used to scale down the bids across all auctions: for any $i, j$, bidder $i$ participates in the auction for good $j$ with a bid equal to $\alpha_i v_{ij}$; we refer to these bids as multiplicatively paced. We call an instance of the above auction market a pacing game. Given a profile of multipliers for a pacing game, $\alpha = (\alpha_1,\dots,\alpha_n)$, we will use $p_j(\alpha)$ to denote the per-unit price of good $j$ given by the pricing rule $p_j$ for the bid profile $(\alpha_1 v_{1j},\dots, \alpha_n v_{nj})$.

\begin{definition}
Given a pacing game $(\{v_{ij}\},\{B_i\},\{p_j\})$, a pacing equilibrium $(\{\alpha_i\}, \{x_{ij}\})$ is defined by values of pacing multipliers $\alpha_i \in [0,1]$ for each bidder and fractions $x_{ij}$ indicating how much of each item j each bidder i receives such that:

\begin{itemize}
	\item For all $j$, $\sum_i x_{ij} \leq 1$ (with equality if there is at least one $i$ with $v_{ij} > 0$). Also, for all $i$ and $j$, $x_{ij} > 0$ implies that $i$'s bid $\alpha_i v_{ij}$ was (possibly tied for) the highest bid on $j$.
	\item For all $i$, $\sum_j x_{ij}p_j(\alpha) \leq B_i$. In addition, if the former inequality is strict, then $\alpha_i = 1$.
	
\end{itemize}
\end{definition} 

\begin{definition}
A pacing game $(\{v_{ij}\},\{B_i\},\{p_j\})$ is a mixed price pacing game if there exist $\lambda_j \in [0,1]$ such that $$p_j(b_1,\dots,b_n)  = \lambda_j FP + (1 - \lambda_j) SP\ \forall j$$ where $FP$ and $SP$ represent the highest and second highest bid among $b_1,\dots,b_n$ respectively. We will call $\{\lambda_j\}$ the mixing parameters. For convenience, we will also denote a MPPG by $(\{v_{ij}\},\{B_i\},\{p_j\},\{\lambda_j\})$.
\end{definition}

\begin{definition}
In a market setting with valuations and budgets $(\{v_{ij}\},\{B_i\})$, a competitive equilibrium $(\{P_j\}$ $\{x_{ij}\})$ consists of a price $P_j$ for every item $j$, and an allocation of items to bidders such that every bidder buys a bundle that maximizes her utility, subject to her budget constraint. That is, bidder $i$'s bundle, consisting of fractions $x_{ij}$ she obtains of each item $j$, must be in $\arg\max_{\{x_{ij}: \sum_{j} x_{ij}P_j \leq B_i\}} \{\sum_j x_{ij}(v_{ij} - P_j)\}$. Additionally every item with a positive price must be fully allocated.
\end{definition} 

\noindent Note that every pacing game defines a unique market setting. Therefore it is well-defined to talk about competitive equilibria in a pacing game.

\begin{theorem}
For every pacing equilibrium $(\{\alpha_i\}, \{x_{ij}\})$ of a MPPG $(\{v_{ij}\},\{B_i\},\{p_j\},\{\lambda_j\})$, there is a competitive equilibrium given by $(\{p_j(\alpha)\}$, $\{x_{ij}\})$.
\end{theorem} 
\begin{proof}
Consider a pacing equilibrium $(\{\alpha_i\}, \{x_{ij}\})$ of a MPPG $(\{\alpha_i\}, \{x_{ij}\}, \{p_j\}, \{\lambda_j\})$. Fix agent $i$. Observe that $x_{ij} = 1$ for all items $j$ such that $\alpha_i v_{ij} > p_j(\alpha)$, since $p_j(\alpha)$ is no less than the second highest bid on item $j$, making agent $i$ the unique highest bidder. Moreover, we also have that $x_{ij} > 0$ for item $j$ only when $i$ is (possibly tied for) the highest bid, i.e. $\alpha_i v_{ij} \geq p_j(\alpha)$. Hence, the following statements hold:
\begin{itemize}
    \item $i$ buys every item for which her bang-per-buck $\frac{v_{ij}}{p_j(\alpha)} > \frac{1}{\alpha_i}$
    \item every item $j$ that she buys has bang-per-buck $\frac{v_{ij}}{p_j(\alpha)} \geq \frac{1}{\alpha_i}$
\end{itemize} 
Also, by the definition of a pacing equilibrium, either $\sum_j x_{ij}p_j(\alpha) = B_i$ or $\alpha_i=1$ (Recall that $\sum_j x_{kj}p_j(\alpha) \leq B_k$ for all agents $k$). Therefore, $x_{ij} \in \arg\max_{\{x_{ij}: \sum_{j} x_{ij}p_j(\alpha) \leq B_i\}} \{\sum_j x_{ij}(v_{ij} - p_j(\alpha))\}$: if $\alpha_i<1$ then they are spending their full budget on optimal items; if $\alpha=1$ then any leftover budget is at least as valuable as any further items they can afford. 

Consider an item $j$ with $p_j(\alpha) > 0$. As $p_j(\alpha)$ is a convex combination of $FP(j)$ and $SP(j)$ (Recall that, $FP(j)$ and $SP(j)$ represent the highest and second highest paced bid on $j$ respectively), we get $FP(j)$ ($= \alpha_i v_{ij}$ for some agent $i$) is greater than $p_j(\alpha)$ and is therefore positive. Hence, there exists agent $i$ with $v_{ij} > 0$. By the definition of a pacing equilibrium, $\sum_i x_{ij} = 1$ for such $j$.
\end{proof}

The following example shows that the assumption that the pacing game is a MPPG is required.\\

\noindent \textbf{Example} Consider a pricing rule $p$ such that $p(b_1,\dots,b_n) < SP(b_1,\dots,b_n)$ for some bidding profile $(b_1,\dots,b_n)$. Then, the pacing game with $n$ bidders and a single good, with $v_{i1} = b_i, B_i = \infty$ for all $i \in [n]$ and pricing rule $p$, has a unique pacing equilibrium given by $\alpha_i = 1 \forall i$, where the good is shared equally by the highest bidders and $p(\alpha) < SP(b_1,\dots,b_n)$. In this case, $(\{p(\alpha)\}$, $\{x_{i1}\})$ is not a competitive equilibrium because in any competitive equilibrium $x_{i1} = 1$ for all bidders $i$ with $v_{i1} > p_1$ and there are at least $2$ such bidders.


\begin{theorem}
For every competitive equilibrium $(\{P_j\}$ $\{x_{ij}\})$ in a market setting with budgets $(\{v_{ij}\},\{B_i\})$, there exist mixing parameters $\lambda_j$ and pacing multipliers $\{\alpha_i\}$ such that the MPPG $(\{v_{ij}\},\{B_i\},\{p_j\},\{\lambda_j\})$ has a pacing equilibrium given by $(\{\alpha_i\}, \{x_{ij}\})$ where $P_j = p_j(\alpha)\ \forall j$.
\end{theorem} 

\begin{proof}
Consider a competitive equilibrium $(\{P_j\}$ $\{x_{ij}\})$. For agents $i$ that buy every item (entirely) for which their valuations strictly exceeded the price, set $\alpha_i \coloneqq 1$. For all other agents $i$, define $\alpha_i \coloneqq max_{\{j : x_{ij} > 0\}} \frac{P_j}{v_{ij}}$ \footnote{Set $\frac{P_j}{v_{ij}} = 0$ when $v_{ij}=0$}. Then, we have $\alpha_i \in [0,1]\ \forall i$ as no agent buys a good at a price strictly greater than her valuation in a competitive equilibrium. Note that by defining the profile of pacing multipliers, $\alpha$, we have specified the bid profile for each good in the pacing game.

Fix item $j$. Let $i$ be an agent such that $x_{ij} > 0$ \footnote{The case where no such agent exists is trivial.}. From the definition of $\alpha_i$, we get that $\alpha_i v_{ij} \geq P_j$. Hence, the highest bid for item $j$, $FP(j)$, is no smaller than $P_j$. Suppose, there exists an agent $i$ such that  $\alpha_i v_{ij} > P_j$ and $x_{ij} < 1$. As $i$ does not buy $j$ entirely even with $v_{ij} > P_j$, by the definition of $\alpha_i$, there exists an item $j^*$ such that $\alpha_i v_{ij^*} = P_{j^*}$. But this leads to a contradiction, as in the competitive equilibrium, $i$ should have bought all of $j$ before buying any of $j^*$. Hence, $\alpha_i v_{ij} > P_j$ implies $x_{ij} = 1$. Therefore, no two bidders can have bids strictly greater than $P_j$. This implies that the second highest bid on $j$, $SP(j)$, is no greater than $P_j$. Define $\lambda_j \in [0,1]$ to be such that $P_j = \lambda_i FP(j) + (1 - \lambda_i) SP(j)$. Observe that the above argument also implies that $x_{ij} > 0$ only if $i$'s bid was (possibly tied for) the highest bid on $j$. Finally, note that if $v_{ij} > 0$, then $\sum_{i} x_{ij} = 1$.
\end{proof}

==> includes.tex <==

\usepackage[margin=1in]{geometry}
%\usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}

%\usepackage{fullpage}

\renewcommand{\familydefault}{ppl}
\renewcommand{\baselinestretch}{1}


\usepackage{varioref}
\usepackage[usenames,svgnames,xcdraw,table]{xcolor}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
\usepackage[backref=page]{hyperref}
\hypersetup{
     colorlinks   = true,
     linkcolor    = DarkBlue, % color of internal links
     urlcolor     = DarkBlue, % color of external links
	 citecolor    = DarkGreen % color of links to bibliography
}
\renewcommand*{\backref}[1]{}
\renewcommand*{\backrefalt}[4]{%
    \ifcase #1 (Not cited.)%
    \or        (Cited on page~#2)%
    \else      (Cited on pages~#2)%
    \fi}
%\usepackage[capitalise,noabbrev]{cleveref}


\usepackage{appendix}

\usepackage{mathtools}
\usepackage{mathrsfs}

\usepackage{algorithmic}

\usepackage{algorithm}
\usepackage{array}

\usepackage[font={small,it}]{caption}
\usepackage{csquotes}




\usepackage{graphicx,epsfig,amsmath,latexsym,amssymb,verbatim}%,revsymb}

%%%%%%%%%%%%%%%%%%%%%
% Handling comments and versions %%%
%%%%%%%%%%%%%%%%%%%%%
\newcommand{\extra}[1]{}

\renewcommand{\comment}[1]{{\color{red}\texttt{[#1]}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{theorem}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{amsthm}
\usepackage{thmtools,thm-restate}
\usepackage{enumitem}

\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}{Claim}
\newtheorem*{remark2}{Remark}

%\theoremstyle{remark}



% Proofs

\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
\def\endenv{\ifmmode\;\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\;
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\renewenvironment{proof}{\noindent \textbf{{Proof~} }}{\qed\medskip}
\newenvironment{proof+}[1]{\noindent \textbf{{Proof #1~} }}{\qed\medskip}
\newenvironment{remark}{\noindent \textit{{Remark.~}}}{\qed}
\newenvironment{example}{\noindent \textbf{{Example~}}}{\qed}

% Align := properly in math mode
\mathchardef\ordinarycolon\mathcode`\:
\mathcode`\:=\string"8000
\def\vcentcolon{\mathrel{\mathop\ordinarycolon}}
\begingroup \catcode`\:=\active
  \lowercase{\endgroup
  \let :\vcentcolon
  }

\mathchardef\mhyphen="2D







==> old_reduction.tex <==
\section{Hardness Results}

In this section, we  consider the problem of computing pacing equilibria and show that it is hard for general pacing games. More precisely, we show that the computational problem of finding $(\delta, \gamma)$-\appe\ is PPAD hard, for small enough $\delta$ and $\gamma$. We do so by demonstrating a reduction from $\epsilon$-NE, i.e, we reduce the problem of finding an $\epsilon$-well-supported mixed strategy Nash Equilibrium in a 0-1 cost bi-matrix game to that of finding an $(\delta, \gamma)$-approximate pacing equilibrium in a pacing game.

The proof for PPAD hardness of computing an $(\delta, \gamma)$-approximate pacing equilibrium is quite involved and contains details that might obfuscate the main ideas underlying the reduction. Instead, to highlight these ideas and motivate our techniques, we first provide a reduction from $\epsilon$-PE to the problem of finding an \emph{exact} pacing equilibrium. Furthermore, for ease of exposition, we first establish the hardness in pacing games which allow for some of the items to be sold through first-price auctions . This forms the content of the first subsection.

\subsection{Hardness of Finding Exact Pacing Equilibria in Games with First Price goods} \label{section_hardness_first_price}

 Consider a 0-1 cost bi-matrix game specified by $n \times n$ cost matrices $(A,B)$. We would like to create a pacing game $\mathcal{I}$ using $(A,B)$ such that every pacing equilibrium in $\mathcal{I}$ can be mapped back to a NE for the bi-matrix game. Then, finding a pacing equilibrium for $\mathcal{I}$ would be at least as hard as finding a NE for the bi-matrix game.
 
 Before proceeding further, we informally describe some important aspects of the reduction to provide some intuition. First, as part of the reduction, we will encode the mixed strategies (probability distributions over pure strategies $[n]$) using pacing variables. For each player $p \in \{1,2\}$ and each strategy $s \in [n]$, there will be a corresponding buyer (called the $(p,s)$-strategy buyer), whose pacing multiplier will encode the probability with which player $p$ plays strategy $s$.
 
  Second, in order to capture the best response condition of NE, we must encode the cost borne by player $p$ when playing a given strategy $s$ against the mixed strategy of the other player. For simplicity, let us focus on $p =1$. We will create an {\em expenditure gadget} for each strategy $s$ of player 1, consisting of $n$ goods (called $E(1,s)_1, \dots, E(1,s)_{n}$). Moreover, we will set the $(1,s)$-strategy buyer's value at 1 for each of the expenditure gadget goods $\{E(1,s)_1, \dots, E(1,s)_{n}\}$. Additionally, the $(2,t)$-strategy buyer will value the expenditure good $E(1,s)_t$ at $\nu A_{st}$, where $\nu$ is so small that the $(1,s)$-strategy buyer always wins all the goods $\{E(1,s)_1, \dots, E(1,s)_{n}\}$ under any pacing equilibrium. This means that, in any pacing equilibrium with multipliers $\alpha(a)$ for buyer $a$, the $(p,s)$-strategy buyer pays a total of $\nu \sum_s \alpha(\S(2,t)) A_{st}$ for the expenditure goods $\{E(1,s)_1, \dots, E(1,s)_{n}\}$, which captures player 1's cost for playing $s$, when player 2 uses the mixed strategy that plays $t$ with probability proportional to $\alpha(\S(2,t))$ (for fully mixed strategies; actions played with probability zero must be handled via thresholding as described next).
  
  Finally, we would also like to make sure that the NE best response condition is satisfied, i.e., only the best response strategies are played with positive probability. This poses a challenge because pacing multipliers are never zero in a pacing equilibrium, so we can't use them directly to encode probabilities (which need to be zero for strategies which are not best responses). To get around this issue, we will use thresholds, calibrated to ensure that a pacing multiplier at this threshold level corresponds to zero probability. We will define {\em threshold goods} and {\em threshold buyers} to help with this calibration.
  
We are now ready to formally define the game $\mathcal{I}$. It has the following set of goods, with each good being a second-price good unless mentioned otherwise:
\begin{itemize}
    \item $(p,s)$-Strategy Gadget: For each player $p \in \{1,2\}$ and strategy $s \in [n]$, there are $n$ strategy goods $\{S(p,s)_1, \dots,  S(p,s)_n\}$, with $S(p,s)_{s}$ being a \textbf{first price good}.
    
    \item $(p,s)$-Threshold Good: For each player $p \in \{1,2\}$ and strategy $s \in [n]$, there is a threshold good $T(p,s)$.
    
    \item $(p,s)$-Expenditure Gadget: For each player $p \in \{1,2\}$ and strategy $s \in [n]$, there are $n$ items $\{E(p,s)_1, \dots, E(p,s)_{n}\}$.
\end{itemize}

Set $\nu = 1/(16n)$. The set of buyers in $\mathcal{I}$ is defined as follows:

\begin{itemize}
    \item $(p,s)$-Strategy Buyer: For each player $p \in \{1,2\}$ and strategy $s \in [n]$, there is a buyer $\mathbb{S}(p,s)$. Buyer $\mathbb{S}(p,s)$ has positive value only for the following goods:
    \begin{itemize}
        \item All $(p,s)$-strategy goods other than $S(p,s)_s$ have value $2$, i.e., $V(\mathbb{S}(p,s), S(p,s)_i) = 2$ for all $i \in [n]\setminus{\{s\}}$.
        
        \item The $s$th $(p,s)$-strategy good has value $1$, i.e., $V(\mathbb{S}(p,s), S(p,s)_s) = 1$.
        
        \item The $s$th $(p,t)$-strategy good at value $1$ for all $t \neq s$, i.e., $V(\mathbb{S}(p,s), S(p,t)_s) = 1$ for all $t \in [n]\setminus \{s\}$.
        
        \item The $(p,s)$-threshold good has value $2n^4$, i.e., $V(\mathbb{S}(p,s), T(p,s)) = 2n^4$
        
        \item All $(p,s)$-expenditure goods $\{E(p,s)_1, \dots, E(p,s)_n\}$ have value $1$, i.e., $V(\mathbb{S}(p,s), E(p,s)_i) = 1$ for all $i \in [n]$.
        
        \item For $p = 1$: $\mathbb{S}(1,s)$ values the $s$th $(2,t)$-expenditure good at $\nu B_{st}$ for all $t \in [n]$, i.e., $V(\mathbb{S}(1,s), E(2,t)_s) = \nu B_{st}$ for all $t \in [n]$.
        
        For $p = 2$: $\mathbb{S}(2,s)$ values the $s$th $(1,t)$-expenditure good at $\nu A_{ts}$ for all $t \in [n]$, i.e., $V(\mathbb{S}(2,s), E(1,t)_s) = \nu A_{ts}$ for all $t \in [n]$.
    \end{itemize}
    For all $s \in [n]$, the budget of $\mathbb{S}(1,s)$ is $n/2 + n^4 + 1/4 + \sum_t \nu A_{st}/2$ and the budget of $\mathbb{S}(2,s)$ is $n/2 + n^4 + 1/4 + \sum_t \nu B_{ts}/2$.
    
    \item Threshold Buyer: There is a restricted buyer $\mathbb{T}$. Buyer $\mathbb{T}$ has positive value only for the following goods:
    \begin{itemize}
        \item For each player $p \in \{1,2\}$ and strategy $s \in [n]$, we have $V(\mathbb{T}, T(p,s)) = n^4$.
        \item For $p=1$: The expenditure good $E(1,s)_t$ has value $\nu A_{st}/2$ for all $s,t \in [n]$.
        
        For $p=2$: The expenditure good $E(2,s)_t$ has value $\nu B_{ts}/2$ for all $s,t \in [n]$.
    \end{itemize}
    
    $\mathbb T$ has an infinite budget (or equivalently she has a budget so large that she is never paced in any pacing equilibrium).
\end{itemize}

Let $\mathscr{E}$ be a pacing equilibrium of the game $\mathcal{I}$. Observe that, from the definition of pacing equilibrium, we can conclude that the pacing multiplier of $\mathbb{T}$ in $\mathscr{E}$ is $1$. We will use $\alpha(a)$ to denote the pacing multiplier of buyer $a$ in $\mathscr{E}$.  The following lemma establishes bounds on the equilibrium pacing multipliers of the strategy buyers.

\begin{lemma}\label{mutlipliers_bounds}
    For each player $p \in \{1,2\}$ and strategy $s \in [n]$, we have $1/2 \leq \alpha(\S(p,s)) <1$.
\end{lemma}

\begin{proof}
    Suppose for some $p \in \{1,2\}$ and $s \in [n]$, we have $\alpha(\S(p,s)) < 1/2$. Then, $\mathbb{S}(p,s)$ doesn't win any part of $T(p,s)$. Observe that she has value at most $2$ for every good in $I$ except $T(p,s)$, and there are at most $n^3$ goods in $\mathcal{I}$. Therefore, the sum of her bids on all items other than $T(p,s)$ is at most $2 n^3$. Hence, she can't possibly spend more than $n^4$. This contradicts the definition of a pacing equilibrium because her budget is strictly greater than $n^4$. Therefore, $(\alpha(\S(p,s)) \geq 1/2$ for each player $p \in \{1,2\}$ and strategy $s \in [n]$.\\
    
    Next, suppose $\alpha(\S(p,s)) = 1$ for some $p \in \{1,2\}$ and $s \in [n]$. Then, she wins the following goods in their entirety:
    \begin{itemize}
        \item Strategy good $S(p,s)_t$ at a price greater or equal to $1/2$ for each $t \in [n] \setminus \{s\}$, because $\alpha(\S(q,r)) \geq 1/2$ for all $p \in \{1,2\}$, $r \in [n]$ by the first part of the proof.
        
        \item Strategy sood $S(p,s)_s$ at a price of $1$ (Recall that this good is a first price good).
        
        \item Threshold good $T(p,s)$ at a price of $n^4$.
        
        \item Expenditure good $E(p,s)_t$ at a price greater than $\nu A_{st}/2$ if $p=1$ and $\nu B_{ts}/2$ if $p=2$.
    \end{itemize}
    Hence, the total expenditure is greater than $(n-1)/2 + 1 + n^4 + \sum_t \nu A_{st}/2$ if $p=1$ and greater than $(n-1)/2 + 1 + n^4 + \sum_t \nu B_{ts}/2$ if $p=2$. In both cases, the budget constraint is violated, leading to a contradiction. Therefore, the lemma holds.
\end{proof}

The above lemma states that the construction of $\mathcal{I}$ ensures that all the strategy buyers are paced in $\mathscr{E}$, thereby implying that their total expenditures must exactly equal their budgets. Next, we define our mapping from equilibrium multipliers to unnormalized mixed strategies for the bi-matrix game. For $s \in [n]$, set $x_s = \alpha(\S(1,s)) - 1/2$ and $y_s = \alpha(\S(2,s)) - 1/2$. The following lemma will allow us to normalize $x$ and $y$ to obtain valid probability distributions.

\begin{lemma} \label{multiplier_positive_sum}
    The following inequalities hold: $\sum_s x_s > 0$ and $\sum_s y_s > 0$.
\end{lemma}

\begin{proof}
    We prove $\sum_s x_s > 0$. The proof of $\sum_s y_s > 0$ is completely analogous. Suppose $\sum_s x_s = 0$. Then, $x_s = 0$ for all $s \in [n]$, or in other words, $\alpha(\S(1,s)) \leq 1/2$ for all $s \in [n]$. By the previous lemma, this implies that $\alpha(\S(1,s)) = 1/2$ for all $s\in [n]$. Therefore, the strategy buyer $\mathbb{S}(1,1)$ only wins a non-zero fraction of the following goods, and spends:
    \begin{itemize}
        \item $1/2$ on strategy good $S(1,1)_t$ for all $t \in [n]$.
        
        \item At most $n^4$ on threshold good $T(1,1)$.
        
        \item At most $\nu A_{1t}$ on Expenditure Good $E(1,1)_t$, for all $t \in [n]$
    \end{itemize}
    Hence, the total expenditure of strategy buyer $\mathbb{S}(1,1)$ is at most $n/2 + n^4 + \sum_t \nu A_{1t}$, which is strictly less than her budget of $n/2 + n^4 + 1/4 + \sum_t \nu A_{st}/2$, thereby contradicting the feasibility of the equilibrium $\mathscr{E}$.
\end{proof}

Now, we are ready to define the mixed strategies for the bi-matrix game corresponding to pacing equilibrium $\mathscr{E}$. Set player 1's mixed strategy to be $\{x_s/ \sum_s x_s\}_s$ and player 2's mixed strategy to be $\{y_s/ \sum_s y_s\}_s$. These are valid mixed strategies because of Lemma \ref{mutlipliers_bounds} and Lemma \ref{multiplier_positive_sum}. To complete the proof of PPAD hardness, we need to show that the mixed strategies defined in this way form a NE for the bi-matrix game, which is the subject of the next lemma.

\begin{lemma}
	$(\{x_s/ \sum_s x_s\}_s, \{y_s/ \sum_s y_s\}_s)$ is a NE for the bimatrix game with cost matrices $(A,B)$.
\end{lemma}

\begin{proof}
	Consider $s \in [n]$ such that $x_s > 0$. Then, $\mathbb{S}(1,s)$ spends non-zero amounts only on the following goods:
\begin{itemize}
    \item $\alpha(\S(1,t))$ on strategy good $S(1,s)_t$ for all $t \in [n]$.
    
    \item $n^4$ on threshold good $T(1,s)$.
    
    \item $\max\{\alpha(2,t), 1/2\} \nu A_{st}$ on $E(1,s)_t$ for all $t \in [n]$.
\end{itemize}

Therefore, the total expenditure of $\mathbb{S}(1,s)$, for buyer $s$ with $x_s> 0$, is given by 
\begin{align*}
    \sum_{t} \alpha(\S(1,t)) + n^4 + \sum_t \max\{\alpha(\S(2,t)), 1/2\} \nu A_{st} = \sum_{t} \alpha(1,t) + n^4  + \sum_t \nu A_{st}/2 + \sum_t y_t \nu A_{st}
\end{align*}

Note that the last term in the total expenditure is proportional to the expected cost incurred by player 1 in the bimatrix game when player 2 uses the mixed strategy $\{y_s/ \sum_s y_s\}_s$. Moreover, the budgets of the buyers differ in a way that neutralizes the differences in the second last term of the above expression. Next, we show that this observation forces strategies $s$ of player 1 which are not best responses to have $x_s = 0$.\\

Let $s^* \in \arg \min_s \sum_t y_t A_{st}$. Suppose there exists $s \in [n]$ such that $x_s > 0$ and $\sum_t y_t A_{st} > \sum_t y_t A_{s^*t}$. Then, by the definition of pacing equilibrium, we have
\begin{align*}
    \sum_{t} \alpha(\S(1,t)) + n^4  + \sum_t \nu A_{st}/2 + \sum_t y_t \nu A_{st} &= n/2 + n^4 + 1/4 + \sum_t \nu A_{st}/2\\
    \implies  n/2 + 1/4 - \sum_{t} \alpha(\S(1,t)) &= \nu \sum_t y_t A_{st} > \nu \sum_t y_t A_{s^*t} \\
    \implies n/2 + n^4 + 1/4 + \sum_t \nu A_{s^*t}/2 &> \sum_{t} \alpha(\S(1,t)) + n^4  + \sum_t \nu A_{s^*t}/2 + \sum_t y_t \nu A_{s^*t}
\end{align*}

In the last inequality, the RHS represents an upper bound on the expenditure of $\mathbb{S}(1,s^*)$ and the LHS is the budget of $\mathbb{S}(1,s^*)$, which contradicts the definition of a pacing equilibrium. Hence, we have shown that
\begin{align*}
    \sum_t \frac{y_t}{\sum_u y_u} A_{st} > \sum_t \frac{y_t}{\sum_u y_u} A_{s^*t} \implies \frac{x_s}{\sum_u x_u} = 0
\end{align*}
which is the required condition for $\{x_s/ \sum_s x_s\}_s$ to be a best response for player 1 when player 2 employs $\{y_s/ \sum_s y_s\}_s$. Similarly, we get that $\{y_s/ \sum_s y_s\}_s$ is a best response for player 2 against the use of $\{x_s/ \sum_s x_s\}_s$ by player 1, thereby completing the proof. 
\end{proof}

\subsection{Mimicking First Price Goods using Second-Price Goods} \label{section_mimic_first-price}

In this subsection, we construct a gadget using second-price goods which mimics the behavior of a single first-price good, which in turn allows us to extend the hardness result of the previous section to finding pacing equilibria in pacing games consisting solely of second-price goods. We begin by specifying how to construct this gadget, and then incorporate it in the reduction of the previous section.

Let $p \in\ \{1,2\}$ and $s \in [n]$. The gadget (we call it the algebra gadget) which will replace the first-price strategy good $\mathbb{S}(p,s)_s$ consists of three algebra goods $\{A_1(p,s), A_2(p,s), A_3(p,s)\}$ and two algebra buyers $\{\A^1(p,s), \A^2(p,s)\}$. Algebra buyer $\A^1(p,s)$ has positive value only for the following goods:
\begin{itemize}
    \item The $1$st algebra good at $4$ and the $3$rd algebra good at $2$, i.e., $V(\A^1(p,s), A_1(p,s)) = 4$ and $V(\A^1(p,s), A_3(p,s)) = 2$.
\end{itemize}
    
Algebra buyer $\A^2(p,s)$ has positive value only for the following goods:
\begin{itemize}
    \item The $2$nd algebra good at $4$ and the $3$rd algebra good at $2$, i.e., $V(\A^2(p,s), A_2(p,s)) = 4$ and $V(\A^2(p,s), A_3(p,s)) = 2$.
\end{itemize}
Both algebra buyers have budget $1$.\\

Add the above gadget to the pacing game $\mathcal{I}$ created in the previous subsection. Furthermore, modify the valuation of $(p,s)$-strategy buyer so that she values the first and second algebra goods at $1/2$ (her valuation for the rest of the goods remains the same). Consider a pacing equilibrium $\mathscr{E}$ of this modified pacing game. Observe that if $\alpha(\A^1(p,s)) \leq 1/8$, then the total payment made by algebra buyer $\mathbb{A}(p,s)$ is at most $1/2 + 1/4$, which is strictly less than her budget. This contradicts the definition of a pacing equilibrium. Hence, $\alpha(\A^1(p,s)) > 1/8$ in $\E$. Moreover, it is easy to see that $\alpha(\A^1(p,s)) = \alpha(\A^2(p,s))$ because otherwise the one with the smaller multiplier would be under-spending in $\E$. It is also straightforward to see that if $\alpha(\A^1(p,s)) = \alpha(\A^2(p,s)) = 1$, then the $(p,s)$-algebra buyer who wins the larger fraction of the third algebra good $A_3(p,s)$ spends more than her budget, which is a contradiction. Hence, $1/8 < \alpha(\A^1(p,s)) = \alpha(\A^2(p,s)) < 1$. As every buyer who is paced must exactly spend her budget in $\E$, we get the following equivalent statements
\begin{align*}
	\frac{1}{2} \cdot \alpha(\mathbb{S}(p,s)) + \frac{1}{2} \cdot 2 \cdot\alpha(\mathbb{A}^t(p,s)) = 1 	\iff \alpha(\mathbb{A}^t(p,s)) = 1 - \frac{1}{2} \cdot \alpha(\mathbb{S}(p,s)) \tag{for $t \in \{1,2\}$}
\end{align*}

Note that, with the help of this algebra gadget, we were able to perform the algebraic operation $x \mapsto 1 - x/2$ with the multiplier $\alpha(\mathbb{S}(p,s))$, i.e., starting from a player with multiplier $\alpha(\mathbb{S}(p,s))$, we have created a buyer with multiplier $1 - \alpha(\mathbb{S}(p,s))/2$. Furthermore, since the strategy buyer $\mathbb{S}(p,s)$ won no item in this algebra gadget, we did not affect her expenditure. Next, we will create another copy of the algebra gadget to achieve the following transformation:
\begin{align*}
	x \mapsto 1 - \frac{1 - x/2}{2} = \frac{x}{4} + \frac{1}{2}	
\end{align*}
With these two copies of the algebra gadget, we can get a buyer with multiplier $\alpha(\mathbb{S}(p,s))/4 + 1/2$. Finally, have this newly created buyer like the $s$th $(p,s)$-strategy good $S(p,s)_s$ at $4$ and change the value that the $(p,s)$-strategy buyer $\mathbb{S}(p,s)$ has for the $(p,s)$-strategy good $S(p,s)_s$ to $16$. Then, this series of changes to $\mathcal{I}$ has the effect of changing the payment of the $\mathbb{S}(p,s)$ for the $(p,s)$-strategy good $S(p,s)_s$ from $\alpha(\mathbb{S}(p,s))$ (when it was a first price good) to $\alpha(\mathbb{S}(p,s)) + 2$. The additional $2$ can be compensated for in the budget of $\mathbb{S}(p,s)$. Therefore, we have successfully mimicked first price goods using second-price goods. The modified pacing game described in this section gives a reduction from the problem of finding NE in bi-matrix games to the problem of finding pacing equilibria in Second Price Pacing Games.

\begin{theorem}\label{exact_hardness}
	Computing exact pacing equilibria in Second Price Pacing Games is PPAD hard. 	
\end{theorem}

We omit the full proof of Theorem \ref{exact_hardness} because it follows directly from Theorem \ref{approximate_hardness}, which we state next, and whose proof can be found in Appendix \ref{appendix_hardness}.



\subsection{Hardness of Finding Approximate Pacing Equilibria} \label{section_approx_hardness}

We are now ready to state our main hardness result, which addresses the computational complexity of finding $(\delta, \gamma)$-approximate pacing equilibria.   

\begin{theorem} \label{approximate_hardness}
	The problem of computing a $\left(\frac{1}{(nm)^2}, \frac{1}{(nm)^2}\right)$-\appe\ of a pacing game $G = (n, m, (v_{ij}),(B_i))$ is PPAD hard.  	
\end{theorem}

The proof of Theorem \ref{approximate_hardness} follows from a modification of the reduction given in subsection \ref{section_hardness_first_price}, which only uses second-price goods (achieved by using the techniques described in subsection \ref{section_mimic_first-price}) and to incorporate the approximations introduced in the definition of $(\delta, \gamma)$-\appe. It entails more involved bookkeeping to keep track of the approximations, which doesn't add much to the reader's intuition, and hence, has been relegated to Appendix \ref{appendix_hardness}.

Before concluding this section, we record some implications of our hardness results. In \cite{borgs2007dynamics}, the authors introduced an extremely natural bidding heuristic for optimizing the utility of budget-constrained agents who repeatedly participate in day-long auction campaigns for $m$ items, where the set of agents and items remains the same every day. The heuristic maintains a pacing multiplier for each agent, which is increased by a small amount if the buyer ran out of her daily budget before the end of the previous day, and decreased otherwise. They use random perturbation to avoid instabilities, which gives an agent who bids close to the highest bid a fraction of the item in expectation. If we ignore the intra-day temporal aspects of their model, their setting can be thought of as repeatedly playing a pacing game every day. In Theorem 1 of \cite{borgs2007dynamics}, they prove that their heuristic efficiently converges for first-price auctions. Furthermore, they conjecture the convergence of the heuristic for second-price auctions to pacing multipliers which satisfy the following conditions: (i) Every agent runs out of her daily-budget close to the end of the day; (ii) Every agent either spends most of her daily budget or has a pacing multiplier close to 1. It can be shown that this is equivalent to convergence to an $(\delta, \gamma)$-\appe\ for the corresponding pacing game, where $\delta$ comes from the definition of the random perturbations and $\gamma$ is the approximation factor used to measure the extent of the convergence. Thus, Theorem~\ref{approximate_hardness} implies that, under standard complexity-theoretic assumptions, the heuristic of \cite{borgs2007dynamics} cannot converge efficiently, i.e., the number of days/time-steps required for convergence cannot scale as a polynomial function of the input size and $(1/\delta, 1/\gamma)$. In other words, we have shown that Theorem 1 of \cite{borgs2007dynamics} cannot be extended to second-price auctions in any way that maintains efficient convergence, thereby making progress towards their open conjecture.

Our hardness result is also pertinent to the relationship between pacing equilibria and market equilibria. In Proposition 5 of \cite{conitzer2017multiplicative}, the authors show that every pacing equilibrium in a second-price pacing game has an equivalent supply-aware market equilibrium in the corresponding Fischer market with linear utilities, where supply-aware means that the buyers are aware of the supplies of each item and choose their demand set accordingly. The concept of supply-aware market equilibria is an extension of the standard notion of market equilibria, in which the buyers select their demand set with no regard for the supply (but the supply constraints need to be satisfied nonetheless). In \cite{conitzer2019pacing}, it is shown that pacing equilibria for first-price auctions correspond to the standard notion of market equilibrium and hence, can be computed efficiently using the Eisenberg-Gale convex program \cite{}. Thus, the relationship between pacing equilibria and market equilibria, in combination with Theorem \ref{approximate_hardness}, implies that there exists a refinement of the set of supply-aware market equilibria which is PPAD hard to compute, even though, in general, a supply-aware market equilibrium can be found in polynomial time using the Eisenberg-Gale program. 


